A joint optimization approach to identifying sparse dynamics using least squares kernel collocation

We develop an all-at-once modeling framework for learning systems of ordinary differential equations (ODE) from scarce, partial, and noisy observations of the states. The proposed methodology amounts to a combination of sparse recovery strategies for the ODE over a function library combined with techniques from reproducing kernel Hilbert space (RKHS) theory for estimating the state and discretizing the ODE. Our numerical experiments reveal that the proposed strategy leads to significant gains in terms of accuracy, sample efficiency, and robustness to noise, both in terms of learning the equation and estimating the unknown states. This work demonstrates capabilities well beyond existing and widely used algorithms while extending the modeling flexibility of other recent developments in equation discovery.

==> numerics.tex <==
\begin{tabularx}{\linewidth}{
  Y
  S[table-format=1.2]
  S[table-format=2.2,table-space-text-post = \%]
  c
  S[scientific-notation=true,round-precision=2]
  S[scientific-notation=true,round-precision=2]
  S[table-format=1.3]
  Y
  S[table-format=3.0]
  Y
  S[table-format=1.2]
  S[table-format=1.2]
  S[scientific-notation=true,table-format=1.0e1]
  S[scientific-notation=true,table-format=1.0e5]
  S[scientific-notation=true,table-format=1.0e-3]
}
\toprule
Exp & {noise} & {Rel.\ \%} & ord & {MSE} & {MAE} & {$\Delta t$} & Obs. & {$t_1$} & Pattern & thr & $\alpha$ & data\_w & colloc\_w & $\beta_{\rm reg}$ \\
\midrule
Scarce Lorenz & 0 & 0.00 & 1 & 2.59e-6 & 1.96e-3 & 0.5 & 21 (*3) & 10 & Full & 0.5 & 0.01 & 1 & 1e5 & 1e-3 \\
Lotka–Volterra & 0.2 & 19.68 & 1 & 1.28e-2 & 2.41e-2 & 3 & 17 (*2) & 50 & Full & 0.1 & 0.1 & 1 & 1e5 & 1e-3 \\
Lorenz Streams & 0.1 & 1.23 & 1 & 3.24e-5 & 1.56e-2 & 0.025 & 404 & 10 & Rotating seg. & 0.25 & 0.01 & 1 & 1e5 & 1e-3 \\
Lorenz Unobs. & 0.1 & 1.26 & 1 & 4.68e-5 & {N/A} & 0.025 & 404 & 10 & 3rd coord. unobs. & 0.1 & 0.01 & 1 & 1e5 & 1e-3 \\
Van der Pol & 0.1 & 7.39 & 2 & 2.06e-3 & 1.69e-1 & 2 & 50 & 100 & Pos.-only & 0.1 & 0.01 & 1 & 1e5 & 1e-3 \\
Coupled Duffing & 0.2 & 16.85 & 2 & 1.26e-3 & 3.07e-2 & 0.2 & 150 (*5) & 30 & Pos.-only & 0.1 & 0.01 & 1 & 1e5 & 1e-3 \\
Nonlin pend. (lin) & 0.1 & 4.17 & 2 & 1.56e-2 & {N/A} & 1 & 100 & 100 & Pos.-only & 0.1 & 0.01 & 1 & 1e5 & 1e-3 \\
Nonlin pend. (cubic) & 0.1 & 4.17 & 2 & 4.93e-4 & {N/A} & 1 & 100 & 100 & Pos.-only & 0.1 & 0.01 & 1 & 1e5 & 1e-3 \\
\bottomrule
\end{tabularx}


==> thmsetup.tex <==
\newtheorem{proposition}{proposition}
